Scalable Deep Metric Learning on Attributed Graphs

We consider the problem of constructing embeddings of large attributed graphs and supporting multiple downstream learning tasks. We develop a graph embedding method, which is based on extending deep metric and unbiased contrastive learning techniques to 1) work with attributed graphs, 2) enabling a mini-batch based approach, and 3) achieving scalability. Based on a multi-class tuplet loss function, we present two algorithms -- DMT for semi-supervised learning and DMAT-i for the unsupervised case. Analyzing our methods, we provide a generalization bound for the downstream node classification task and for the first time relate tuplet loss to contrastive learning. Through extensive experiments, we show high scalability of representation construction, and in applying the method for three downstream tasks (node clustering, node classification, and link prediction) better consistency over any single existing method.

==> input/related_work.tex <==
\vspace*{-2ex} 
\section{Related Work}
\vspace*{-2ex} 


% \subsection{Summary of references from the reviewers:}
% \begin{enumerate}
%    \item CGML~\cite{chen2021_graph_consistency} proposed a graph-based relation modeling on image classification.
%    \item SUBG-CON~\cite{jiao2020_sub} a scalable framework focuses on node classification. 
%    \item  SCGC~\cite{liu2022_SCGC} (source code not accessible): dedicated for node clustering and only reports results for this single task. 
%    \item DCRN~\cite{liu2022_deep} only for node clustering, buggy code not runnable. 
%    \item A graph debiased contrastive learning model ~\cite{zhao2021_graph}, for node classification and clustering. incomplete code not runnable.
%     \item ProGCL~\cite{xia2022_progcl} is based on ~\cite{zhu2021_GCA} by adding couple of lines in their models. Only for node classification. 
% \end{enumerate}


\noindent\textbf{Attributed Graph Representation Learning.}
Graph Autoencoder (GAE) based models \cite{kipf2016variational_VGAE,Pan_2018_AVGAE,wang_mgae_2017}  learn 
node embeddings that can recover either node features or the adjacency matrix. 
%through their  architectures. 
Adaptive Graph Convolution (AGC) \cite{ijcai2019_AGC}   uses high-order graph convolution to capture global cluster structure and adaptively selects   the appropriate order for different graphs. Simple Spectral Graph Convolution (SSGC)  \cite{ssgc_2021}  is a variant of GCN that  exploits a modified Markov Diffusion Kernel.  Adaptive Graph Encoder (AGE) \cite{Cui_AGE_2020} combines a customized Laplacian smoothing filter with an adaptive encoder  to strengthen the filtered features for better node embeddings. In using GCN modules for node clustering,
SDCN~\cite{Bo_2020_structural_deep} is a 
self-supervised method. 
\cite{zhao2021_graph} proposed a graph debiased contrastive learning approach to jointly perform representation learning and clustering. GCA~\cite{zhu2021_GCA} is a graph contrastive
representation learning method with adaptive augmentation. ProGCL~\cite{xia2022_progcl} boosts the graph contrastive learning by estimating the probability of a negative being true. DCRN~\cite{liu2022_deep} improves the representation discriminative capability for node clustering by reducing information correlation. 


\noindent\textbf{Deep Metric Learning.} 
%As mentioned previously, here one trains the networks to learn  feature embeddings where similar examples are mapped close to each other and dissimilar examples are mapped farther apart. 
\cite{bromley_1993_signature} laid the foundation of this area motivated by 
signature verification. \cite{chopra_2005_learning} discriminatively trains the network for face verification via contrastive loss, \cite{Schroff_2015_FaceNetAU} learns a unified embedding for face clustering and recognition through triplet loss, and 
\cite{cui_2016_fine} focuses on  visual categorization. \cite{Sohn_N-pair_loss_objective_2016} proposed (N+1)-tuplet loss for a variety of visual recognition tasks. \cite{yoshida_2021_distance} proposes a supervised distance metric learning for graph classification. 
It should be noted that  the contrastive loss here aims to ensure that the distance between examples from different classes is larger than a certain margin~\cite{Sohn_N-pair_loss_objective_2016}. 
The methods we next discuss under constrastive learning have a different emphasis. 
%which is different from the concept as defined in contrastive learning as introduced in the following. 


\noindent\textbf{Contrastive Learning.}
As one major branch of self-supervised learning, contrastive learning, 
when combined with augmentation techniques,  has achieved state-of-the-art performance in visual representation learning tasks~\cite{oord_2019_representation,hjelm_2019_DIM,Tian_multi_coding_2020,chen_simple_framework_contastive_2020,contrastiveLoss_wu2018}. This idea has also been applied for node-level representation learning for graph-structured data~\cite{velickovic_2019_DGI,zhu2021_GCA}. Deep Graph Infomax (DGI) \cite{velickovic_2019_DGI} achieves advanced node classification performance by extending  a contrastive learning mechanism (from precursor work Deep InfoMax~\cite{hjelm_2019_DIM}). 
GCA~\cite{zhu2021_GCA} applied the contrastive loss from~\cite{chen_simple_framework_contastive_2020} to maximize agreements at the node level and performed well on node classification tasks.  
We later discuss how our approach differs and also perform  extensive experimental comparison. 

% Several efforts have been made to demystify contrasting mechanism~\cite{TscDjoRubGelLuc_On_mutual_2020,Ben_good_view_CL_2020,Wu2020OnMI,wang_2020_hypersphere}, however, the reason behind the success of contrastive learning still remains unclear.

% Several efforts have also been made to demystify the success of contrastive learning. \cite{Ben_good_view_CL_2020} argued that view selection depends on the downstream task and the mutual information (MI) between views should be reduced while keeping task-relevant information intact. %  where data augmentation is considered to be one way of decreasing MI. 
% \cite{Wu2020OnMI} provides a mutual information framework to compare between different contrastive learning approaches and highlights the importance of negative sampling and view selection. \cite{TscDjoRubGelLuc_On_mutual_2020} empirically argued that MI properties alone cannot explain the success of these methods and the biased encoder and MI estimator played an important role. \cite{wang_2020_hypersphere} identified two properties,  alignment and uniformity, that contrastive loss asymptotically optimized. Another research~\cite{wang_2021_CL_behavior} shows that contrastive loss is hardness-aware and the hyper-paremter temperature $\tau$ controls the strength of penalties on hard negative samples. 




